Fairness Properties of Face Recognition and Obfuscation Systems

The proliferation of automated face recognition in the commercial and government sectors has caused significant privacy concerns for individuals. One approach to address these privacy concerns is to employ evasion attacks against the metric embedding networks powering face recognition systems: Face obfuscation systems generate imperceptibly perturbed images that cause face recognition systems to misidentify the user. Perturbed faces are generated on metric embedding networks, which are known to be unfair in the context of face recognition. A question of demographic fairness naturally follows: are there demographic disparities in face obfuscation system performance? We answer this question with an analytical and empirical exploration of recent face obfuscation systems. Metric embedding networks are found to be demographically aware: face embeddings are clustered by demographic. We show how this clustering behavior leads to reduced face obfuscation utility for faces in minority groups. An intuitive analytical model yields insight into these phenomena.

==> src_usenix/225_Face_Obfuscation.tex <==
 
\section{Face Obfuscation}
\label{sec:faceObfuscation}

Researchers have demonstrated that systems which leverage principles from adversarial machine learning can provide users with privacy utility in the presence of face recognition systems.  These privacy benefits are encapsulated in systems known as face obfuscation systems. In this section, we present the notation and discuss the work relevant to such face obfuscation systems.

\subsection{Threat Model}
\label{subsec:threat}
 In the face obfuscation setting, an end user considers the machine learning provider to be the main threat. They wish to apply (imperceptible) perturbations to their faces, prior to uploading them, so that the presence of faces are correctly recognized, but the predicted identity of faces is incorrect. Such protection might be beneficial in the event of social media data leaks~\cite{holmes2021facebook}, preventing cyber-stalking~\cite{harwell_2021}, protecting data from web scrapers, hiding online activity from big government entities~\cite{Goodwin_2021}, and more.
% https://www.gao.gov/products/gao-21-105309

State-of-the-art designs for face obfuscation systems leverage evasion attacks.  Such attacks were described in \cref{subsec:AdvMachineLearning}. Unlike other attacks, evasion attacks assume the user is not able to poison the face recognition system. An important property of adversarial examples, especially for vision tasks such as face recognition, is their ability to transfer across models.  This property allows users to generate adversarial examples without requiring access to an online face recognition API and without directly querying said model. Instead, face obfuscation systems leverage this properties by querying surrogate models to generate the perturbed faces. In a \textit{white-box} setting, examples are generated with the intention of attacking the surrogate model. In the \textit{black-box} setting, examples are generated on the surrogate model and applied to a black-box model, by leveraging the transferability property. 


\subsection{Face Obfuscation Systems}

The earliest work in this vein of face obfuscation research explores physical adversarial examples. For example, Sharif et al.~\cite{sharif2016glasses} present physically realizable glasses that allow a human user to impersonate a target individual and evade face detection systems. Recently, there has been a shift in focus towards preserving user privacy online from malicious web scrappers, data breaches, and intrusive service providers. Thus, researchers have focused more on digital face obfuscation systems, which are more suited for social media and online applications.  Examples of such systems include FAWKES~\cite{DBLP:Fawkes}, Face-Off~\cite{DBLP:FaceOff}, Low-Key~\cite{DBLP:LowKey}, and FoggySight~\cite{evtimov21foggysight}. With the exception of FAWKES, which leverages data poisoning attacks, these face obfuscation systems utilize evasion attacks with an attempt to hide the user's identity. These systems are the main focus of this paper.

We now describe these face obfuscation systems more formally. Let $\getPerturbation$ denote an evasion attack function (e.g. PGD, CW), and let $\perturbation$ denote a generic perturbation output by the evasion attack function, i.e. $\getPerturbation(\sample)$. A face obfuscation system feeds $\sample + \perturbation$ into the face recognition system.  Note that perturbaton function $\getPerturbation$ may include dependence on the metric embedding network, the underlying dataset, or some other surrogate model.  
% Throughout this work, we explore how these face obfuscation systems fare for each demographic under a variety of adversarial attack algorithms.

\subsection{Evasion Attacks on Face Recognition}
\label{subsec:Adversarial}

 Evasion attacks may be divided into targeted and untargeted varieties.  To define the two attacks, we first describe the embedding centroid.  Given a dataset $\trainingData$, denote by $\centroid_{\embeddingFunc,\labelElement}$ the embedding centroid for identity $\labelElement$ as computed on embedding function $\embeddingFunc$ is:
{\small 
\begin{equation}
    \centroid_{\embeddingFunc,\labelElement} \definedAs \frac{1}{\abs{\left\{(\sample',\labelElement') \in \trainingData  \given \labelElement' = y \right\}}}\sum_{(\sample',\labelElement')\in \trainingData} \embeddingFunc(\sample')\cdot\indicatorFunction\left[\labelElement' = y\right]
\end{equation}
}

% Given a classifier $\classifier$, loss function $\ell$ and projection function $\Pi$, the $(t+1)^{\mathrm{th}}$ step of the PGD attack may be written as:
% \begin{align}\label{eq:PGD}
% (\sample)^{t+1}=\Pi_{x+S}(x^{t}+\alpha\cdot\sgn(\nabla_{x}L(\theta,x,y)))
% \end{align}

% The Carlini-Wagner $\ell_2$ attack\cite{carlini17wagner} uses an outer optimization loop which bounds the $\ell_2$ norm of the generated perturbation.  Given an adversarial evasion attack  It is defined as the following:
% \begin{align}\label{eq:CW1}
% \min{\left\Vert \dfrac{1}{2}(\tanh(w)+1)-x\right\Vert^{2}_{2}+c \cdot f(\dfrac{1}{2}(\tanh(w)+1))}
% \end{align}
% where f is defined as
% \begin{align*}\label{eq:CW2}
% f(x')=\max(\max{\{Z(x')_{i}:i \neq t\}}-Z(x')_{t},-\kappa)
% \end{align*}

% The previous equations are formulations for a classification setting. Since face recognition adopts metric embedding networks, below are general adversarial attack formulations for the metric learning setting.


\noindent \textbf{Untargeted Attacks:}
Recall from \cref{subsec:notation} that a metric $\metric$ given only one explicit argument is assumed to have a size-conforming zero vector as its second argument. Given a metric embedding network $\embeddingFunc: \sampleSpace \to \labelSpace$,  unlabeled example $\sample$, and metrics $\metric_1,\metric_2$ an \emph{untargeted attack} may be formulated as:
{\small
\begin{align}
\begin{gathered}
  \min_{\perturbation \given \sample + \perturbation\in \sampleSpace}  \metric_1 (\perturbation)\\
  \textrm{s.t.}  \argmin_{\labelElement' \in \labelSpace} \metric_2(\centroid_{\embeddingFunc,\labelElement'},\embeddingFunc(\sample))  
     \neq \argmin_{\labelElement' \in \labelSpace} \metric_2(\centroid_{\embeddingFunc,\labelElement'},\embeddingFunc(\sample + \perturbation))
%   \textrm{s.t.} \quad &\argmin_{j \in [k]} \phi (\beta_{c_j,f},f_\theta()) \neq  \argmin_{j \in [k]} \phi (\beta_{c_j,f},f_\theta(+\delta))
\end{gathered} 
\label{eq:untargetedAttack}
\end{align}
}

The problem with the formulation above is that the constraint is non-convex.  To make the attack implementable in practice, the constraints must be relaxed.  For a labeled example $(\sample,\labelElement)$, the optimization objective which yields an untargeted perturbation can be written as:
{\small
\begin{align}
\begin{split}
\label{eq:untar_lowkey}
\argmax_{\perturbation \given \sample' + \perturbation \in \sampleSpace}  \metric_2(\embeddingFunc(\sample'+\perturbation),\centroid_{\embeddingFunc,\labelElement}) \; \;
\textrm{s.t.} \; \; \metric_1(\perturbation) \leq \epsilon
\end{split}
\end{align}
}

In this paper, we use the LowKey attack~\cite{DBLP:LowKey} to instantiate \cref{eq:untar_lowkey}. In this case, PGD is use to solve the optimization problem, $\metric_1$ is the Learned Perceptual Image Patch Similarity (LPIPS) metric~\cite{zhang2018lpips}, and  $\metric_2$ is the distance between the original face and perturbed face in the embedding space. Note that the latter distance is averaged through an ensemble of models and after applying Gaussian smoothing.  



\noindent \textbf{Targeted Attacks:}  
Given a target label $\labelElement'$, metric embedding network $\embeddingFunc: \sampleSpace \to \labelSpace$,  unlabeled example $\sample$, and metrics $\metric_1,\metric_2$ a \emph{targeted attack} may be formulated as follows:
{\small
\begin{align}
\begin{split}
  \min_{\perturbation \given \sample + \perturbation\in \sampleSpace}  \metric_1 (\perturbation) \;
  \textrm{s.t.} \; \labelElement' = \argmin_{\labelElement \in \labelSpace} \metric_2(\centroid_{\embeddingFunc,\labelElement},\embeddingFunc(\sample + \perturbation))
%   \textrm{s.t.} \quad &\argmin_{j \in [k]} \phi (\beta_{c_j,f},f_\theta()) \neq  \argmin_{j \in [k]} \phi (\beta_{c_j,f},f_\theta(+\delta))
\end{split}\label{eq:targetedAttack}
\end{align}
}

Similar to the untargeted case, attacks on face recognition systems relax the above constraints to arrive at a convex optimization formulation. Here, we state one such relaxation from Face-Off~\cite{DBLP:FaceOff}, which we use in the rest of this paper.  First, we define the multi-class hinge loss.  The multi-class hinge loss enables a convex relaxation of the constraints in the targeted attack \cref{eq:targetedAttack}.  Given a perturbed example $\sample + \perturbation$, target label $\labelElement'$, and positive real number $\kappa$, the multi-class hinge loss is denoted by $\hinge_{\kappa}(\sample + \perturbation, \labelElement')$ where: 
{\small
\begin{align}
\begin{gathered}
    \hinge_{\kappa}(\sample+\perturbation,\labelElement') \definedAs \max\Big\{0,\kappa+\metric_2(\sample+\perturbation, \centroid_{\embeddingFunc,\labelElement'})\\ \qquad-\max_{\labelElement \neq \labelElement'}\metric_2(\sample+\perturbation, \centroid_{\embeddingFunc,\labelElement})\Big\}
\end{gathered}
\end{align}
}

For a labeled example $(\sample,\labelElement)$, and target label $\labelElement' \neq \labelElement$, the CW attack can minimize the following optimization objective:
{\small
\begin{equation}
\label{eq:face-off}
\argmin_{\perturbation \given \sample + \perturbation \in \sampleSpace}  \metric_1(\perturbation) \;
\textrm{s.t.} \; \metric_1(\perturbation) \leq \epsilon \;
\textrm{and} \;  \hinge_{\kappa}(\sample + \perturbation,\labelElement') \leq 0
\end{equation}
}

% Given an embedding function $\embeddingFunc: \realNumbers^{\dimension} \to \realNumbers^k$, embedding space metric $\metric_2$, and reference dataset $\trainingData$. Define:

% \begin{equation}
%     \metric_2'({\embeddingFunc(\sample,\trainingData_{\labelElement = \labelElement_0})}) \definedAs \frac{1}{\abs{\trainingData_{\labelElement = \labelElement_0}}} \sum_{(\sample',\labelElement)\in \trainingData_{\labelElement = \labelElement_0}} {\metric_2(\embeddingFunc(\sample),\embeddingFunc(\sample'))}
% \end{equation}












% \subsection{Implementing Adversarial Attacks for Facial Recognition}
% %%Kassem: make sure if do not redefine variables, and use variables from previous sections if possible.
% % Chandrasekaran et al in Face-Off~\cite{DBLP:FaceOff}.

% The previous section describes evasion attacks in the targeted (\cref{eq:targetedAttack}) and untargeted (\cref{eq:untargetedAttack}) settings, but has a fundamental flaw: In the following, we describe the constrained employed in practice, preceded with some notation. 






% We focus our study on evasion attacks, where an adversary generates an adversarial example, subject to some constraints, that changes the classification output at inference time.
% The vast majority of research involving adversarial machine learning take the perspective of a  user whose goal is to maximize the accuracy of a machine learning model to which the user has access.  In such a setting, evasion attacks, such as those generated by Projected Gradient Descent (PGD)~\cite{madry2017towards}, are assumed to be perpetrated by adversarial actors.  These attacks can be used to fool malware detection, impersonate identities, inject hidden commands, and more. Unlike the canonical machine learning setting, the setting of this work considers the machine learning provider to be the main threat.  A pertinent example of machine learning used by an adversary is an Orwellian Big Brother-esque surveillance state \cite{Orwell1984}.  

% Such scenarios include preserving privacy in the event of social media data leaks~\cite{holmes2021facebook}, preventing cyber-stalking\cite{} \harrison{@brian do you know of a good reference on this one?}, protecting data from web scrapers, hiding online activity from big government entities~\cite{greenwald_2013,swan_2021}, and more.  Under the cloud of such surveillance, evasion attacks are seen instead as useful privacy preservation tools.  Hence, the adversarial actor we are considering is the entity operating a facial recognition system, and our goal is to subvert this surveillance state's ability to operate an accurate facial recognition system, while still being able to upload photos online.




%  on machine learning systems mesh well with those who wish to subvert facial recognition systems.  The design of face obfuscation systems, which are intended to thwart privacy incursions by face recognition systems, constitutes a relatively recent research vein. 


% As machine learning sees increasingly prevalent usage in our society, researchers have since then explored several properties of adversarial examples such as physical realizability\cite{}, transferability across models\cite{}, and robustness vs. natural accuracy trade-offs\cite{}.  




% Traditionally, evasion attacks such as Projected Gradient Descent\cite{madry2017towards}, Fast Gradient Sign Method\cite{goodfellow2014explaining}, and the Carlini-Wagner Attack \cite{carlini2017towards} are employed to maliciously attack a classification model (See Section~\ref{subsec:Adversarial}). Face obfuscation systems flip the script by leveraging the ability of such evasion attacks in an effort to limit privacy and security incursions from facial recognition providers.

% By uploading targeted adversarial examples, FoggySight allows privacy guarantees for these target individuals.

% In the commercial sector, a chatbot-based legal firm known as DoNotPay has added a face obfuscation tool, to their app\cite{vincent2021donotpay} in a push for consumer privacy. It is imperative we fully understand the fairness implications of using face obfuscation systems before jumping into widespread adoption.  

==> src_usenix/250_High_Level.tex <==
% \section{High Level Overview}

\noindent
\subsection{RoadMap} 
The rest of this paper consists of three major components: analytical analysis of a simple embedding model, empirical characterization of face recognition and demographic disparities, and an empirical evaluation of the performance of face obfuscation. \textbf{\Cref{sec:theory}} provides an intuitive analytical model based on a simple, theoretically tractable embedding: Principal Component Analysis (PCA).  We study the PCA applied to Gaussian mixtures which are designed to simulate embeddings of face recognition datasets. In\textbf{ \cref{sec:methodology}}, we follow by characterizing the performance of face recognition systems when conditioned on the sex and race attributes. We investigate the dependence of face recognition on demographic attributes through t-SNE~\cite{maaten2008tsne} and TCAV scores~\cite{kim18tcav}. Then, we study the stability of the networks for samples from different demographics using estimates of the local Lipschitz constants. Finally, we conduct an empirical analysis of face obfuscation in \textbf{\cref{sec:experiments}}, for both targeted and untargeted settings. We find the size of the perturbation, success rate, and distribution of targets to depend on the demographic attributes of the source face.




==> src_usenix/275_Theory.tex <==
\section{Analytical Model}\label{sec:theory}
To understand the fairness issues associated with face recognition and obfuscation, we present a tractable, simplified model on synthetic data. This model is inspired by the hierarchical nature of popular face recognition datasets.  The synthetic data consists of examples drawn from a parametrized hierarchical Gaussian mixture we define in \cref{subsec:theorySetup}. We use a $k$-component PCA as an embedding function -- a PCA embedding function which only utilizes projections onto the leading $k$ principal components to perform its dimensionality reduction -- because it is useful for our analysis.  Such analysis is common in the space of  machine learning. Though all samples drawn from our simplified model are vectors, we use the terms \emph{identity} and \emph{image} to draw parallels between the hierarchical nature of our probabalistic model and the hierarchical structure of existing face recognition datasets.   
% Our example highlights the impact of data imbalances which can affect fairness properties of both face obfuscation and face recognition systems. 
% Before delving into conclusions we may draw from our simplified model, we describe the data distribution itself.
\subsection{Setup}\label{subsec:theorySetup}


Similar to empirical datasets, we analyze our synthetic dataset by conditioning on a simulated demographic group. Within the dataset, there are two mutually exclusive population groups: group $\groupA$ and group $\groupB$.  We sometimes use a placeholder $\placeholderGroup$ to represent a group $\placeholderGroup \in \left\{\groupA,\groupB\right\}$. The mean vector for population groups $\groupA$ and $\groupB$ are denoted by $\vec{\mu}_{\groupA} \in \realNumbers^{\dimension}$ and $\vec{\mu}_{\groupB} \in \realNumbers^{\dimension}$, respectively. Moreover, $\vec{\mu}_{\groupA} = -\vec{\mu}_{\groupB}$, $\norm{\vec{\mu}_{\groupA}}_2 = 1$, and $\norm{\vec{\mu}_{\groupB}}_2 = 1$. 

The $i^{\mathrm{th}}$ identity in group $\placeholderGroup$ is denoted by $\vec{\nu}_{\placeholderGroup,i} \in \realNumbers^{\dimension}$.  The $j^{\mathrm{th}}$ image representing identity $\vec{\nu}_{\placeholderGroup,i}$ is denoted by $\sample_{\placeholderGroup,i,j} \in \realNumbers^\dimension$.  $\vec{\Sigma}_{\groupA} \in \realNumbers^{\dimension \times \dimension}$ and $\vec{\Sigma}_{\groupB}\in \realNumbers^{\dimension \times \dimension}$ are diagonal covariance matrices. Furthermore, $\vec{\Sigma}_{\groupA} = \gamma\vec{\Sigma}_{\groupB}$ where $\gamma$ is a positive, real-valued scalar.
An identity $\vec{\nu}_{\placeholderGroup,i}$ is drawn from the identity distribution $\normalDist(\vec{\mu}_{\placeholderGroup},\vec{\Sigma}_{\placeholderGroup})$.  The identity distribution may be thought of as a hyperprior on images. An image $\sample_{\placeholderGroup,i,j}$ is drawn from $\normalDist(\vec{\nu}_{\placeholderGroup,i}, \beta \vec{I})$ where $\beta$ is a positive, real-valued number. Moreover, for each identity $\vec{\nu}_{\placeholderGroup,i}$, exactly $\placeholderCount$ images are drawn from $\normalDist(\vec{\nu}_{\placeholderGroup,i}, \beta \vec{I})$.  Lastly, we denote by $\sampleDist_{\placeholderGroup}$ the distribution of images in group $\placeholderGroup$. 

The synthetic data distribution is a linear combination of image distributions for group $\groupA$ ($\sampleDist_{\groupA}$) and group $\groupB$ ($\sampleDist_{\groupB}$).  Let $\alpha_{\groupA} \in [0,1]$ denote the proportion of examples drawn from group $\groupA$ and let $\alpha_{\groupB} \in [0,1]$ denote the proportion of examples drawn from $\groupB$. Since the population groups are mutually exclusive, we know $\alpha_{\groupA} + \alpha_{\groupB} = 1$.  The synthetic data distribution, we denote by $\sampleDist$ is a linear combination , that is $\sampleDist = \alpha_{\groupA}\sampleDist_{\groupA} + \alpha_{\groupB}\sampleDist_{\groupB}$. We denote by $\trainingData$ a sampling of images  drawn from $\sampleDist$.

\subsection{The Ideal Embedding Function}

In the context of machine learning, an ideal embedding function $\embeddingFunc_k : \realNumbers^{\dimension} \to \realNumbers^{k}$ is one which preserves distances within a dataset. While this property is important for face recognition and obfuscation, it is not the only consequential property of embedding functions.  In the context of fair face recognition, we concern ourselves with how well the embedding represents a particular group from the lens of that group.  For $k$ component PCA, we introduce a quantity, called the relative projection distance, which captures this concept.


\begin{definition}
Let $\trainingData$ be a sample of images drawn from the overall synthetic distribution $\sampleDist$.  The relative projection distance of a point $\sample$, a member of group $\placeholderGroup$, with respect to the leading $k$ principal components of a dataset $\trainingData$ is denoted by $\metric_{\rp, \trainingData,\placeholderGroup,k}: \sampleSpace \to \realNumbers^+$.  More precisely, the quantity is defined as:
{\small
\begin{equation}
\label{eq:relative_proj_dist}
    \metric_{\rp, \trainingData,\placeholderGroup,k}(\sample) \definedAs \frac{\norm{\left(\sample-\sum_{i=1}^{k}\left\{\frac{\vec{q}_i^\transpose \sample}{\norm{\vec{q}_i}_2 \norm{\sample}_2}\vec{q}_i\right\}\right)}_2}{\sum_{j=1}^{\dimension}\left(\vec{\Sigma}_{\placeholderGroup}\right)_{jj}},
\end{equation}
}
where the eigen-decomposition of the covariance of overall synthetic data distribution $\sampleDist$ is  $\vec{\Sigma} = \vec{Q}\vec{\Lambda}\vec{Q}^{\transpose}$.  Furthermore, $\vec{Q}$ may be decomposed as $\vec{Q} = \left[\vec{q}_1,\dotsc,\vec{q}_\dimension\right]^\transpose$.
\end{definition}

Let us explain the reasoning behind this formulation of the relative projection distance.  The numerator computes the norm of the portion of sample $\sample$ which is orthogonal to the subspace spanned by the first $k$ principal components of sample $\trainingData$ drawn from $\sampleDist$.  This portion of $\sample$ is also known as an error vector.   The denominator represents a group specific normalization factor.  This normalization factor represents the total variance within the identity vectors  $\left\{\vec{\nu}_{\placeholderGroup,1}, \vec{\nu}_{\placeholderGroup,2},\dotsc,\right\}$ of group $\placeholderGroup$.  It is this normalization factor which allows us to show how error can be measured through the lens of each group.  In summary, the relative projection distance captures the error induced by the embedding function, as measured through the lens of only population group $\placeholderGroup$.  


% Similar to empirical datasets, we analyze our synthetic dataset by conditioning on the simulated demographic groups. Within the dataset, there are two mutually exclusive population groups: group $\groupA$ and group $\groupB$.  We use a placeholder $\placeholderGroup$ to represent $\placeholderGroup \in \left\{\groupA,\groupB\right\}$. The underlying data distribution $\sampleDist$, is a hierarchical Gaussian mixture which has overall covariance matrix $\vec{\Sigma}_{Y}$.  Identities in group $\placeholderGroup$ are sampled from  $\normalDist(\vec{\mu}_{\placeholderGroup},\vec{\Sigma}_{\placeholderGroup,Y})$.  For real valued $\beta,\gamma > 0$, we assume $\vec{\mu}_{\groupB} = -\vec{\mu}_{\groupA}$, $\norm{\vec{\mu}_{\groupA}}_2 = 1$, $\norm{\vec{\mu}_{\groupB}}_2 = 1$ and $\vec{\Sigma}_{\groupB,Y} = \gamma \vec{\Sigma}_{\groupA,Y}$, where both $\vec{\Sigma}_{\groupA,Y}, \vec{\Sigma}_{\groupB,Y}$ are diagonal matrices, though $\vec{\Sigma}_{Y}$ is not necessarily diagonal. $\numSamples_{\placeholderGroup}$ denotes the number of identities in group $\placeholderGroup$.  Individual identities in group $\placeholderGroup$  are denoted $(i, \placeholderGroup)$, where $i \in \left\{1,\dotsc,\numSamples_{\placeholderGroup}\right\}$.
% Denote the mean parameter for the $i^{\textrm{th}}$ identity in group $\placeholderGroup$ by $\vec{\mu}_{i,\placeholderGroup}$.   Images representing identity $i_{\placeholderGroup}$ are then sampled from $\normalDist(\mu_{\placeholderGroup,i},\beta\vec{I})$ where $\beta$ is a positive, real-valued scalar and $\vec{I}$ is a size-conforming identity matrix.  Exactly $\placeholderCount$ images are drawn for each identity.  Though all samples drawn from our simplified model are random Gaussian vectors, we use the terms \emph{identity} and \emph{image} to draw parallels between the hierarchical nature of our Gaussian mixture and hierarchical structure of existing face recognition datasets.  
    % ratio = distance.cosine(pca.components_[0],x)
    % cosine_distance_ratio.append(distance.cosine(ratio,x))
    % perpendicular_distance.append((ratio*np.linalg.norm(x)))
    % perpendicular_distance_ratio.append(ratio*np.linalg.norm(x)/(gamma_a*S[0]))

% Let us now introduce terminology used to discuss the efficacy of embedding functions. To do so, we introduce the \emph{relative projection distance}.  


% \begin{definition}
% The relative projection distance of a point $\sample$ sampled from group $\placeholderGroup$ with respect to the leading $k$ principal components of training $\trainingData$ is denoted by $\metric_{\rp, \sampleDist,\placeholderGroup,k}: \sampleSpace \to \realNumbers^+$.  More precisely, the quantity is defined as

% \begin{equation}
%     \metric_{\rp, \trainingData,\placeholderGroup,k}(\sample) \definedAs \sum_{i=1}^{k}\frac{\left(1-\frac{\abs{\vec{q}_i^\transpose \sample}}{\norm{\vec{q}_i}_2 \norm{\sample}_2}\right)\norm{\sample}_2}{\sum_{j=1}^{k}\vec{\Lambda}_{\placeholderGroup,jj}}
% \end{equation}

% where the eigen-decomposition of the overall covariance is  $\vec{\Sigma}_Y = \vec{Q}\vec{\Lambda}\vec{Q}^{\transpose}$ and the eigen-decomposition of the covariance matrix for group $\placeholderGroup$ is $\vec{\Sigma}_Y = \vec{Q}_\placeholderGroup\vec{\Lambda}_{\placeholderGroup}\vec{Q}^{\transpose}_\placeholderGroup$
% \end{definition}

% When the training set is clear from context, we omit its subscript.  Intuitively, the relative projection distance captures the error induced by the embedding function, as measured through the lens of only one population group.  

% The relative projection distance is similar in spirit to norm of the error vector in the Graham-Schmidt orthonormalization process.  The primary difference being that the relative projection distance includes a division by the leading eigenvalue of the group $\placeholderGroup$ $\sampleDist_{\placeholderGroup}$ covariance matrix whereas the Graham-Schmidt process does not contain such division.


% The relative projection distance tells us how well (or faithfully) an embedding function represents an image.  We say an embedding $\faithfulParameter$-faithfully represents an image in group $\placeholderGroup$ if its expected relative projection distance $\metric_{\rp, \trainingData,\placeholderGroup,k}$ is less than $\faithfulParameter$, where $\faithfulParameter$ is a positive, real-valued number. That is to say an embedding $\faithfulParameter$-faithfully represents group $\placeholderGroup$ if
% \begin{equation}
% \E_{\sample \drawnFrom \sampleDist_{\placeholderGroup}} \left[\metric_{\rp, \trainingData,\placeholderGroup,k}\right] \leq \faithfulParameter
% \end{equation}

% Similarly, an embedding $\faithfulParameter$-faithfully represents an example $\sample$ in group $\placeholderGroup$ if

% \begin{equation}
% \metric_{\rp, \trainingData,\placeholderGroup,k}(\sample) \leq \faithfulParameter
% \end{equation}

% The parameter $\faithfulParameter$ captures how well the embedding represents a given face image $\sample$.  The lower the value of $\faithfulParameter$, the more faithful the embedding.    Intuitively, for a given image $\sample$, a less-faithful embedding is more susceptible to evasion attack.   In experiments on our analytical model, we observe that images drawn from different groups may have values of $\faithfulParameter$ which differ by orders of magnitude.   This is further demonstrated in \cref{fig:plotRelProjectionDistance}, which contains plots of the relative projection distance for PCA trained on several synthetic datasets. This observation is consistent with our findings in \cref{sec:experiments}, where we find that face recognition networks are less stable for faces sampled from minority groups.
% Intuitively, a faithful representation occurs when the distance between a sample $\sample$, and its projection onto the first $k$ principal components is small.  
% Conversely, a less faithful embedding means a higher value of the faithful parameter $\faithfulParameter$.

% If this is not true, we say the embedding does not faithfully represent group $\placeholderGroup$.
\subsection{Instantiating the Embedding Function}\label{subsec:InstantiateEmbedding}


Let us now instantiate our synthetic distribution with a $k$-component PCA as the embedding function $\embeddingFunc_k$. Utilization of this embedding function enables us to show how relative projection distance may vary greatly between demographic groups $\groupA$ and $\groupB$.  \Cref{fig:plotRelProjectionDistance} depicts how the distribution of relative projection distances induced by $\embeddingFunc_k$ may be either equal or disparate when conditioning by population group. For a demographic group, the distribution of relative projection distance depends on how much a population group contributes to the covariance $\vec{\Sigma}$ of the overall data distribution $\sampleDist$. The contribution to covariance is measured by the \emph{covariance contribution}.  For our synthetic data distribution $\sampleDist$, we compute the covariance contribution from population group $\placeholderGroup$ as:
{\small
\begin{equation}
\label{eq:cov_cont}
    \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\placeholderGroup})_{ii}\right),
\end{equation}
}
where $k$ is the number of principal components used in the PCA embedding and $\vec{\Sigma}_{\placeholderGroup}$ is the covariance matrix for the group $\placeholderGroup$ identity distribution.  

From our understanding of the synthetic data distribution developed by decomposition of $\vec{\Sigma}$ detailed in \cref{subsec:covarianceDecomposition}, we now put forth a proposition regarding the distribution of relative projection distance amongst examples in each group.  

\begin{proposition}\label{prop:relProjectionDistance}
    For a population group $\placeholderGroup$, as the covariance contribution (defined in \cref{eq:cov_cont}) increases, the relative projection distance (defined in \cref{eq:relative_proj_dist}) decreases.
\end{proposition}

Note that increases in covariance contribution may come from increasing the number of samples in population group $\placeholderGroup$ or by increasing the magnitude of covariance $\vec{\Sigma}_{\placeholderGroup}$.

Upon examining the \cref{fig:pca_imbalance,fig:pca_balance}, proposition~\ref{prop:relProjectionDistance} holds true:  In both subfigures, there are 2500 identities per group, making $\alpha_{\groupA} = \alpha_{\groupB} = 0.5$.  Further, there are  $\placeholderCount = 50$ images sampled per identity.    In \cref{fig:pca_balance}, both groups have identical covariance matrices, but in \cref{fig:pca_imbalance}, $\frac{1}{10000}\vec{\Sigma}_{\groupA} = \vec{\Sigma}_{\groupB}$.  

These plots follow the intuition of our proposition exactly: In \cref{fig:pca_balance}, the covariance contributions from each group are equal, hence the distribution of relative projection distance is approximately equal for both groups. In \cref{fig:pca_imbalance}, group $\groupB$ has a much smaller covariance contribution than does group $\groupA$, hence the distribution of relative projection distance for examples within group $\groupB$ is shifted right.




\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/PCA_new_imbalance.png}
         \caption{Relative projection distance is plotted for groups $\groupA$ and $\groupB$ with imbalanced covariance contributions.}
         \label{fig:pca_imbalance}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/PCA_new_balance.png}
         \caption{Relative projection distance is plotted for groups $\groupA$ and $\groupB$ with balanced covariance contributions.}
         \label{fig:pca_balance}
     \end{subfigure}
        \caption{Relative projection distance is plotted for both balanced and imbalanced population groups.}
        \label{fig:plotRelProjectionDistance}
\end{figure}





% \subsection{Embedding Representation}
% Within our  we identify two regimes which capture the behavior of an embedding with respect to (im)balances that occur between demographic groups.  We represent these regimes by changing the conditional distributions for both $\groupA$ ($\sampleDist_{\groupA}$) and $\groupB$ ($\sampleDist_{\groupB}$).  Let $\alpha_{\groupA} \in [0,1]$ denote the proportion of examples drawn from group $\groupA$ and let $\alpha_{\groupB}$ denote the proportion of examples drawn from $\groupB$. Since the population groups are mutually exclusive, we know $\alpha_{\groupA} + \alpha_{\groupB} = 1$.  We formulate a proposition which relates how faithful images are represented to their contribution to overall covariance $\vec{\Sigma}_{\labelElement}$.  



% \begin{proposition}
% Consider a sample $\trainingData$ drawn from our hierarchical Gaussian distribution $\sampleDist$, and let $\embeddingFunc$ be a hierarchical classifier trained on sample $\trainingData$.  Within group $\placeholderGroup$, as $\frac{\alpha_{\placeholderGroup}\norm{\vec{\Sigma}_{\placeholderGroup,Y}}_F^2}{\norm{\vec{\Sigma}_{Y}}_F^2 }$ increases, the PCA embedding function $\embeddingFunc$ tends to more faithfully represent images in group $\placeholderGroup$.
% \end{proposition}

% Moving forward, we utilize the term covariance contribution.  We measure the covariance contribution as the proportion of Frobenius norm contributed by a group $\placeholderGroup$ to the Frobenius norm of covariance matrix $\vec{\Sigma}_Y$ of the overall hierarchical Gaussian distribution.  That is to say, the covariance contribution of group $\placeholderGroup$ is $\frac{\norm{\vec{\Sigma}_{\placeholderGroup,Y}}_F^2}{\norm{\vec{\Sigma}_{Y}}_F^2 }$.

% \subsubsection{Balanced Regime}
% In the balanced regime, each group contributes approximately equally to the overall covariance $\vec{\Sigma}_{Y}$; there are two extremes to discuss:

% % faithfully represents images in both demographic groups
% \noindent
% \textbf{Faithful Representation:}
% The embedding created by PCA on all examples can faithfully represent images in both group $\groupA$, $\groupB$.  This occurs when both demographic groups together make the majority contribution to overall covariance $\vec{\Sigma}_{Y}$.
% {\small
%     \begin{equation}\label{eq:balance_faithful}
%         \begin{split}
%         \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right) \gg 4(1-\alpha_{\groupA}) \;
%         \text{and} \; \left(\beta + \gamma\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right)   \gg 4\alpha_{\groupA}
%         \end{split}
%     \end{equation}
% }
%         \Cref{fig:pca_balance_dominating_1} and \cref{fig:pca_balance_dominating_2}  show how the embeddings trained on all data $\faithfulParameter$-faithfully represents both groups, for a small positive integer $\faithfulParameter$.  In \cref{fig:pca_balance_dominating_1}, the number of examples in each group are equal and the covariance matrices for each group are equal. In  \cref{fig:pca_balance_dominating_2} the number of, the number of examples in each group are equal, but $\vec{\Sigma}_{\groupA} = 100\vec{\Sigma}_{\groupB}$.  When examining the two figures, we see the population group (\cref{fig:pca_balance_dominating_2} with highest covariance has the lowest relative distance.
        
% %  PCA faithfully represent images from neither demographic group}
% \noindent
% \textbf{Unfaithful Representation:}
% The embedding created by PCA on all examples does not faithfully represent images in either demographic group.  This occurs when both demographic groups together make only a very small contribution to overall covariance $\vec{\Sigma}_{Y}$.
% {\small
% \begin{equation}\label{eq:balance_unfaithful}
%         \begin{split}
%         \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right) \ll 4(1-\alpha_{\groupA}) \;
%         \text{and} \; \left(\beta + \gamma\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right)   \ll 4\alpha_{\groupA}
%         \end{split}
%     \end{equation}
%     }
%     \Cref{fig:pca_balance_dominated_1} shows how the embedding trained on only one population group $\faithfulParameter$-faithfully represents both groups, for a small positive integer $\faithfulParameter$.
% %%% ^^^ Are we sure the figure reference is correct??

% \subsubsection{Imbalanced Regime}
% In the imbalanced regime, group $\groupA$ and group $\groupB$ make vastly different contributions to the overall covariance.  Typically, these differential contributions to covariance arise due to numerical imbalance between groups. That is to say the number of examples in group $\groupA$ is much larger than the number of examples in group $\groupB$, or vice versa.  This is not the only source of imbalance.  If the number of examples in group $\groupA$ and group $\groupB$ are equal, vast differences in conditional covariance also constitute imbalance.  In the context of our PCA example, disparities in conditional covariance are captured by $\abs{\log \gamma}$.   Images in the group with larger covariance contribution are more faithfully represented by the PCA embedding.  For group~$\groupA$, this occurs when:
% {\small
%     \begin{equation}\label{eq:imbalance}
%         \begin{split}
%         \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right) \gg 4(1-\alpha_{\groupA}) \;
%         \text{and} \; \left(\beta + \gamma\sum_{i=1}^k(\vec{\Sigma}_{\groupB})_{ii}\right)   \ll 4\alpha_{\groupA}
%         \end{split}
%     \end{equation}
%     }
%     A similar condition can be derived for when group~$\groupB$ makes the larger contribution to overall covariance. Within our decomposition of the overall covariance $\vec{\Sigma}_{Y}$ matrix for scenarios \cref{eq:groupAContribute}, we see that the population group with smaller contribution to covariance suffers from a less faithful representation than the population group which has the larger contribution to covariance.  We see this even when $\vec{\Sigma}_{\groupA} = \vec{\Sigma}_\groupB$  This is demonstrated in \cref{fig:pca_balance_dominating_2}.

%     % or 
%     % {\small
%     % \begin{equation}\label{eq:groupBContribute}
%     %     \begin{split}
%     %     \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right) \ll 4(1-\alpha) \;
%     %     \text{and} \; \left(\beta + \gamma\sum_{i=1}^k(\vec{\Sigma}_{\groupB})_{ii}\right)   \gg 4\alpha
%     %     \end{split}
%     % \end{equation}
%     % }


% \textbf{Regime 2:}   The embedding created by PCA faithfully represents neither group only if PCA was trained on only group $\groupA$ $\sampleDist_{\groupA}$ or only group $\groupB$ $\sampleDist_{\groupB}$.  This occurs when 
% \begin{equation}\label{eq:dominated}
%         \begin{split}
%         \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right) \ll 4(1-\alpha) \\
%         \text{and} \left(\beta + \gamma\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right)   \ll 4\alpha
%         \end{split}
%     \end{equation}
%     \Cref{fig:pca_balance_dominated_1} shows how the embedding trained on only one population group $\faithfulParameter$-faithfully represents both groups, for a small positive integer $\faithfulParameter$.

% \noindent
% \textbf{Regime 3:} The embedding created by PCA faithfully represent either group upon which it was trained. Furthermore, if PCA is trained on data from both groups, then it represents only the group which contributes more variance to the overall data distribution $\sampleDist$.  This occurs when either
%     \begin{equation}\label{eq:groupAContribute}
%         \begin{split}
%         \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right) \gg 4(1-\alpha) \\
%         \text{and} \left(\beta + \gamma\sum_{i=1}^k(\vec{\Sigma}_{\groupB})_{ii}\right)   \ll 4\alpha
%         \end{split}
%     \end{equation}
%     or 
%     \begin{equation}\label{eq:groupBContribute}
%         \begin{split}
%         \left(\beta+\sum_{i=1}^k(\vec{\Sigma}_{\groupA})_{ii}\right) \ll 4(1-\alpha) \\
%         \text{and} \left(\beta + \gamma\sum_{i=1}^k(\vec{\Sigma}_{\groupB})_{ii}\right)   \gg 4\alpha
%         \end{split}
%     \end{equation}
    
%     In \cref{eq:groupAContribute}, group $\groupA$ contributes much more variance to the entire data distribution.  In \cref{eq:groupBContribute}, group $\groupB$ contributes much more variance to the entire data distribution.  \Cref{fig:pca_imbalance} shows how the embedding $\faithfulParameter$-faithfully represents only one population group, where $\faithfulParameter$ is a small positive integer.
    
    
% \end{itemize}

% \begin{figure*}[h]
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/pca_plots/balance_dominating/histogram_rel_distance.png}
%          \caption{$y=x$}
%          \label{fig:pca_balance_dominating}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/pca_plots/balance_dominated/histogram_rel_distance.png}
%          \caption{$y=3sinx$}
%          \label{fig:pca_balance_dominated}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/pca_plots/imbalance/histogram_rel_distance.png}
%          \caption{$y=5/x$}
%          \label{fig:pca_imbalance}
%      \end{subfigure}
%         \caption{We plot the distance between a datapoint and its projection in units of each group's leading covariance term.}
%         \label{fig:three graphs}
% \end{figure*}

% \subsection{A less faithful representation for smaller groups}



\subsection{Connection to Face Obfuscation}\label{subsec:theoryFaceObfuscationConnection}

% To connect our theory to face obfuscation, we discuss the construction of evasion attacks in our analytical model.  Denote by $\PDF_{\placeholderDist}$ the probability density function for probability distribution $\placeholderDist$. Given an example $\sample$, define the maximum likelihood estimator $\MLE(\sample) = \argmax_{\placeholderGroup \in \left\{\groupA,\groupB\right\}} \PDF_{\sampleDist_{\placeholderGroup}}(\sample)$.

% Given an example image $\sample$ in group $\placeholderGroup$, we study how difficult it is to construct a perturbation $\perturbation$ such that $\MLE(\sample + \perturbation) \neq \placeholderGroup$. The synthetic data distribution described in this section is a natural medium with which to quantify the necessary strength of such a perturbation $\perturbation$:

Let $\embeddingFunc : \realNumbers^{\dimension} \to \realNumbers$ be a PCA embedding function. Consider a sample $\sample$ drawn from the overall synthetic data distribution $\sampleDist$ and without loss of generality assume this $\sample$ is a member of group $\groupA$. Assume  $\gamma \leq 1$ , $\PDF_{\sampleDist_{\groupA}}[\vec{\mu}_{\groupA}] > \PDF_{\sampleDist_{\groupB}}[\vec{\mu}_{\groupA}] $, and $\PDF_{\sampleDist_{\groupB}}[\vec{\mu}_{\groupB}] > \PDF_{\sampleDist_{\groupA}}[\vec{\mu}_{\groupB}] $.  Given an adversarial perturbation $\perturbation$, we assume that perturbation $\perturbation$ is norm-bounded and in the direction $\frac{(\vec{\mu}_{\groupB}-\sample)}{\norm{\vec{\mu}_{\groupB}-\sample}_2}$ as it is known to be an adversarial direction. That is, we assume $\norm{\perturbation}_2 \leq \epsilon$ where $\epsilon$ is a non-negative real number.

To capture how strong this perturbation $\perturbation$ can be $\MLE(\sample + \perturbation)$ remains $\groupA$, we quantify the values of $\epsilon$ for which the following optimization problem is guaranteed to be infeasible.  If the optimization problem is infeasible then it is guaranteed that $\MLE(\sample + \perturbation) = \groupA$:


% To connect our theory to face obfuscation, we discuss the construction of evasion attacks in our analytical model.  Consider a sample $\sample$ drawn from the overall synthetic data distribution $\sampleDist$ let $\Pr$ represent a probability density function. Given an adversarial perturbation $\perturbation$, we assume that perturbation $\perturbation$ is norm-bounded.  That is, we assume $\norm{\perturbation}_2 \leq \epsilon$ where $\epsilon>0$ is a non-negative real number.  Without loss of generality assume this $\sample$ is a member of group $\groupA$. Our interest lies in bounding $\zeta^*$ where

% {\small
% \begin{align}
% \begin{split}
% \zeta^* = \min_{\delta : \delta \leq \epsilon} \quad &  \abs{\delta} \\ 
% \mathrm{s.t.} \quad& \Pr_{\sampleElement \drawnFrom \sampleDist_{\groupB}}\left[\sampleElement + \delta\right] >  \Pr_{\sampleElement \drawnFrom\sampleDist_{\groupA}}\left[\sampleElement + \delta \right] \\
% \end{split}
% \end{align}
% }

{\small
\begin{align}
\begin{split}
\min_{\perturbation : \norm{\perturbation}_2 \leq \epsilon} \quad &  \norm{\perturbation}_2 \\ 
\mathrm{s.t.} \quad& \Pr_{\embeddingFunc(\sample) \drawnFrom \sampleDist_{\groupB}}\left[\embeddingFunc(\sample + \perturbation)\right] >  \Pr_{\sample \drawnFrom\sampleDist_{\groupA}}\left[\embeddingFunc(\sample + \perturbation)\right] \\
\perturbation \quad& = \eta \cdot  \frac{(\vec{\mu}_{\groupB}-\sample)}{\norm{\vec{\mu}_{\groupB}-\sample}_2} \text{ where } \eta \in \realNumbers
\end{split} \label{eq:theoryOptimizationProblem}
\end{align}
}

For notational compactness, we denote:
{\small
\begin{align*}
a=\embeddingFunc(\sample) \; \; \text{and} \; \;
b=\embeddingFunc\left(\frac{(\vec{\mu}_{\groupB}-\sample)}{\norm{\vec{\mu}_{\groupB}-\sample}_2}\right).
\end{align*}
}
This optimization objective in \cref{eq:theoryOptimizationProblem} guaranteed to be infeasible when: 
{\small
\begin{equation}
    \epsilon < \max\left\{0,\frac{2b(\gamma-1)\sqrt{\frac{a^2\gamma}{b^2(\gamma-1)^2}} +a\gamma +a + \embeddingFunc(\vec{\mu}_{\groupB})(1-\gamma)}{b(\gamma-1)}\right\} \label{eq:theoryCondition}
\end{equation}\label{eq:optimizationInfeasible}
}
This result is further detailed in \cref{subsec:pcaAdversarialAttack}.


Therefore we conclude that $\MLE(\sample + \perturbation) = \groupA$ when inequality \eqref{eq:optimizationInfeasible} holds.
Furthermore, note that the bound in inequality \eqref{eq:theoryCondition} is not tight, as it becomes more loose as $\gamma$ approaches $0$. Within \cref{eq:optimizationInfeasible}, we notice that for a fixed $\sample$ for which $\MLE(\sample) = \groupA$, as $\gamma$ approaches $0$, the set of perturbations $\perturbation$ for which $\MLE(\sample + \perturbation) = \groupA$ increases in size.  We conclude that as the variation within group $\groupB$ decreases, the embeddings of samples within group $\groupB$ tend to cluster. Hence, pushing a fixed sample in group $\groupA$ to register as a sample in $\groupB$ becomes more difficult for a face obfuscation system. The relevance of this result will be evident later in \cref{sec:methodology,sec:experiments}. The embeddings of faces from minority groups tend to be more concentrated, and we observe that is hard to launch targeted obfuscation towards these groups.





% This result indicates, that for a member of a certain group, a adversarial example will remain in the same population group if not sufficiently strong. The importance of this result lies in its connection to face obfuscation. We find that if faces are clustered in the embedding space according to their demographic attributes, an evasion attack will result in perturbed faces in the same group as the source face. We empirically verify this observation in two steps. \cref{sec:methodology} shows that faces are indeed clustered according to demographic attributes and \cref{sec:experiments} shows that adversarially perturbed faces belong to the same group as the source face. 


% \Cref{fig:pca_balance_dominated_2}  shows that for population groups with small contribution to the covariance matrix, relative to the contribution to covariance by the separation of groups $\groupA$ and $\groupB$. \brian{transition from this to experiments is weird}


% More formally, we have $\sampleDist_{\groupA}=\normalDist(\vec{\mu},\sigma^2\vec{I})$, $\sampleDist_{\groupB}=\normalDist(\vec{\mu}+\vec{\mu}_0,\sigma^2\vec{I})$, and, for some scalar $\alpha \in [0,1]$ $\sampleDist = \alpha \sampleDist_{\groupA} + (1-\alpha)\sampleDist_{\groupB}$.  Our simplified problem is as follows:  Suppose there are $\numSamples_{\groupA}$ samples drawn i.i.d. from $\sampleDist_\groupA$ and an additional $\numSamples_{\groupB}$ samples are drawn i.i.d. from $\sampleDist_{\groupB}$ where $\numSamples_{\groupA} > \numSamples_{\groupB}$.  Draw a new example from $\sampleDist_{\groupB}$. How likely is it for this example to have its nearest neighbor be drawn from $\sampleDist_\groupA$?




% Let $Y$ denote a random variable sampled from the simplified Gaussian Model described in in \cref{sec:theory}.  We also denote the following: $Y_{\groupA}$ and $Y_{\groupB}$ are the random variables representing draws from the identity distributions for group $\groupA$ and group $\groupB$,respectively.  The random variable $Y_{\cdot,i}$ denotes images sampled from the distribution for the $i^{\textrm{th}}$ identity in group $\cdot$.  More formally, we have $Y_{\groupA} \drawnFrom \underbrace{\normalDist(\vec{\mu}_{\groupA},\vec{\Sigma}_{\groupA})}_{\sampleDist_{\groupA}}, Y_{\groupB} \drawnFrom \underbrace{\normalDist(\vec{\mu}_{\groupB},\vec{\Sigma}_{\groupB})}_{\sampleDist_{\groupB}}$, and for all identities $(\cdot,i)$, we have $Y_{\cdot,i} \drawnFrom \underbrace{\normalDist(\vec{\mu}_{\cdot,i},\beta\vec{I})}_{\sampleDist_{\cdot,i}}$

% $\normalDist(\vec{\mu}_{\groupA},\vec{\Sigma}_{\groupA})$ and $\normalDist(\vec{\mu}_{\groupB},\vec{\Sigma}_{\groupB})$, respectively. 
% Denote the mean parameter for the $\cdot,i^{\textrm{th}}$ identity ($\cdot$ is either $\groupA$ or $\groupB$) by $\mu_{\cdot,i}$. Images representing identity $i_{\cdot}$ are then sampled from $\normalDist(\mu_{\cdot,i},\beta\vec{I})$.

% Let $\vec{\mu}_{\groupA}=-\vec{\mu}_{\groupA}$




% To answer this question, we will analyze the distribution of squared Euclidian distance between a sample drawn from $\normalDist(\vec{\mu}-\frac{1}{2}\vec{\mu}_0,\sigma^2\vec{I})$ and another drawn from $\normalDist(\vec{\mu}+\frac{1}{2}\vec{\mu}_0,\sigma^2\vec{I})$.  This distribution is the noncentral chi-squared distribution.  Tail bounds for the noncentral chi square distribution were developed by Birge  {\cite[Lemma~8.1]{Birge2001AnAP}}:

% \begin{lemma}[Tail bounds for Noncentral Chi Square Distribution {\cite[Lemma~8.1]{Birge2001AnAP}}]

% Let $X$ be a noncentral $\chi^2$ random variable with $D$ degrees of freedom and non-centrality parameter $B^{1/2} \geq 0$, then for all $\placeholder > 0$

% \begin{equation}
%     \Pr\left[\placeholderRandomVariable \geq (D + B) + 2\sqrt{(D+2B)\placeholder}+2\placeholder\right] \leq \exp(-\placeholder)
% \end{equation}
% and
% \begin{equation}
%     \Pr\left[\placeholderRandomVariable \geq (D + B) - 2\sqrt{(D+2B)\placeholder}\right] \leq \exp(-\placeholder)
% \end{equation}
% \end{lemma}
